Hierarchical Overlapping Belief Estimation by Structured Matrix Factorization

Much work on social media opinion polarization focuses on a flat categorization of stances (or orthogonal beliefs) of different communities from media traces. We extend in this work in two important respects. First, we detect not only points of disagreement between communities, but also points of agreement. In other words, we estimate community beliefs in the presence of overlap. Second, in lieu of flat categorization, we consider hierarchical belief estimation, where communities might be hierarchically divided. For example, two opposing parties might disagree on core issues, but within a party, despite agreement on fundamentals, disagreement might occur on further details. We call the resulting combined problem a hierarchical overlapping belief estimation problem. To solve it, this paper develops a new class of unsupervised Non-negative Matrix Factorization (NMF) algorithms, we call Belief Structured Matrix Factorization (BSMF). Our proposed unsupervised algorithm captures both the latent belief intersections and dissimilarities, as well as a hierarchical structure. We discuss the properties of the algorithm and evaluate it on both synthetic and real-world datasets. In the synthetic dataset, our model reduces error by 40%. In real Twitter traces, it improves accuracy by around 10%. The model also achieves 96.08% self-consistency in a sanity check.

==> refer.tex <==
\begin{thebibliography}{00}
	\bibitem{b1} Lee, Daniel D., and H. Sebastian Seung. "Algorithms for non-negative matrix factorization." Advances in neural information processing systems. 2001.
	\bibitem{b2} Grčar, Miha, et al. "Data sparsity issues in the collaborative filtering framework." International Workshop on Knowledge Discovery on the Web. Springer, Berlin, Heidelberg, 2005.
	\bibitem{b3} Billsus, Daniel, and Michael J. Pazzani. "Learning Collaborative Information Filters." Icml. Vol. 98. 1998.
	\bibitem{b4} Lancichinetti, Andrea, Santo Fortunato, and Filippo Radicchi. "Benchmark graphs for testing community detection algorithms." Physical review E 78.4 (2008): 046110.
	\bibitem{b5} Al Amin, Md Tanvir, et al. "Unveiling polarization in social networks: A matrix factorization approach." IEEE INFOCOM 2017-IEEE Conference on Computer Communications. IEEE, 2017.
	\bibitem{b6} Fortunato, Santo, and Darko Hric. "Community detection in networks: A user guide." Physics reports 659 (2016): 1-44.
	\bibitem{b7} Yoo, Jiho, and Seungjin Choi. "Orthogonal nonnegative matrix tri-factorization for co-clustering: Multiplicative updates on stiefel manifolds." Information processing and management 46.5 (2010): 559-570.
	\bibitem{b8} Wang, Yu-Xiong, and Yu-Jin Zhang. "Nonnegative matrix factorization: A comprehensive review." IEEE Transactions on Knowledge and Data Engineering 25.6 (2012): 1336-1353.
	\bibitem{b9}  (2016, Jul) Sentiment140 - A Twitter Sentiment Analysis Tool.
	[Online]. Available: http://www.sentiment140.com
	\bibitem{b10} Zhou, Dengyong, Jiayuan Huang, and Bernhard Schölkopf. "Learning with hypergraphs: Clustering, classification, and embedding." Advances in neural information processing systems. 2007.
	\bibitem{b11} Li, Pan, and Olgica Milenkovic. "Inhomogeneous hypergraph clustering with applications." Advances in Neural Information Processing Systems. 2017.
	\bibitem{b12} Bakshy, Eytan, Solomon Messing, and Lada A. Adamic. "Exposure to ideologically diverse news and opinion on Facebook." Science 348.6239 (2015): 1130-1132.
	\bibitem{b13} Bessi, Alessandro, et al. "Users polarization on facebook and youtube." PloS one 11.8 (2016): e0159641.
	\bibitem{b14} Sunstein, Cass R. "The law of group polarization." Journal of political philosophy 10.2 (2002): 175-195.
	\bibitem{b15} Akoglu, Leman. "Quantifying political polarity based on bipartite opinion networks." Eighth International AAAI Conference on Weblogs and Social Media. 2014.
	\bibitem{b16} Conover, Michael D., et al. "Political polarization on twitter." Fifth international AAAI conference on weblogs and social media. 2011.
	\bibitem{b17} Guerra, Pedro Calais, et al. "A measure of polarization on social media networks based on community boundaries." Seventh International AAAI Conference on Weblogs and Social Media. 2013.
	\bibitem{b18} Matakos, Antonis, Evimaria Terzi, and Panayiotis Tsaparas. "Measuring and moderating opinion polarization in social networks." Data Mining and Knowledge Discovery 31.5 (2017): 1480-1505.
	\bibitem{b19} Tian, Leimin, Catherine Lai, and Johanna D. Moore. "Polarity and intensity: the two aspects of sentiment analysis." arXiv preprint arXiv:1807.01466 (2018).
	\bibitem{b20} Musco, Cameron, Christopher Musco, and Charalampos E. Tsourakakis. "Minimizing polarization and disagreement in social networks." Proceedings of the 2018 World Wide Web Conference. International World Wide Web Conferences Steering Committee, 2018.
	\bibitem{b21} Liu, Bing. "Sentiment analysis and opinion mining." Synthesis lectures on human language technologies 5.1 (2012): 1-167.
	\bibitem{b22} Altafini, Claudio. "Dynamics of opinion forming in structurally balanced social networks." PloS one 7.6 (2012): e38135.
	\bibitem{b23} Paatero, Pentti, and Unto Tapper. "Positive matrix factorization: A non‐negative factor model with optimal utilization of error estimates of data values." Environmetrics 5.2 (1994): 111-126.
	\bibitem{b24} A. Cichocki, R. Zdunek, A. Phan, and S. Amari, Nonnegative Matrix and Tensor Factorizations: Applications to Exploratory Multi-Way Data Analysis and Blind Source Separation. John Wiley \& Sons, 2009.
	\bibitem{b25} I. Buciu, “Non-Negative Matrix Factorization, a New Tool for Feature Extraction: Theory and Applications,” Int’l J. Computers, Comm. and Control, vol. 3, pp. 67-74, 2008.
	\bibitem{b26} S. Sra and I. Dhillon, “Nonnegative Matrix Approximation: Algorithms and Applications,” technical report, Univ. of Texas, http://www.cs.utexas.edu/ftp/ftp/pub/techreports/tr06-27. pdf, 2006.
	\bibitem{b27} I. Ulbrich, M. Canagaratna, Q. Zhang, D. Worsnop, and J. Jimenez, “Interpretation of Organic Components from Positive Matrix Factorization of Aerosol Mass Spectrometric Data,” Atmospheric Chemistry and Physics, vol. 9, pp. 2891-2918, 2009.
	\bibitem{b28} K. Drakakis, S. Rickard, R. de Fr' in, and A. Cichocki, “Analysis of Financial Data Using Non-Negative Matrix Factorization,” Int’l Math. Forum, vol. 3, no. 38, pp. 1853-1870, 2008.
	\bibitem{b29} D. Donoho and V. Stodden, “When Does Non-Negative Matrix Factorization Give a Correct Decomposition into Parts?” Proc. Advances in Neural Information Processing Systems, pp. 1141-1148, 2004.
	\bibitem{b30} B. Klingenberg, J. Curry, and A. Dougherty, “Non-Negative Matrix Factorization: Ill-Posedness and a Geometric Algorithm,” Pattern Recognition, vol. 42, no. 5, pp. 918-928, 2009.
	\bibitem{b31} S. Moussaoui, D. Brie, and J. Idier, “Non-Negative Source Separation: Range of Admissible Solutions and Conditions for the Uniqueness of the Solution,” Proc. IEEE Int’l Conf. Acoustics, Speech, and Signal Processing, vol. 5, pp. 289-292, 2005.
	\bibitem{b32}  H. Laurberg, M. Christensen, M. Plumbley, L. Hansen, and S. Jensen, “Theorems on Positive Data: On the Uniqueness of NMF,” Computational Intelligence and Neuroscience, vol. 2008, article ID 764206, doi:10.1155/2008/764206, 2008.
	\bibitem{b33} N. Mohammadiha and A. Leijon, “Nonnegative Matrix Factoriza- tion Using Projected Gradient Algorithms with Sparseness Constraints,” Proc. IEEE Int’l Symp. Signal Processing and Informa-
	tion Technology, pp. 418-423, 2009.
	\bibitem{b34} P. Hoyer, “Non-Negative Matrix Factorization with Sparseness Constraints,” J. Machine Learning Research, vol. 5, no. 9, pp. 1457-
	1469, 2004.
	\bibitem{b35} Lee, Daniel D., and H. Sebastian Seung. "Learning the parts of objects by non-negative matrix factorization." Nature 401.6755 (1999): 788.
	\bibitem{b36} J. Yoo and S. Choi, “Orthogonal Nonnegative Matrix Tri- Factorization for Co-Clustering: Multiplicative Updates on Stiefel Manifolds,” Information Processing and Management, vol. 46, no. 5, pp. 559-570, 2010.
	\bibitem{b37} D. Cai, X. He, J. Han, and T. Huang, “Graph Regularized Non- Negative Matrix Factorization for Data Representation,” IEEE Trans. Pattern Anal. Mach. Intell., vol. 33, no. 8, pp. 1548-1560, Aug. 2011.
	\bibitem{b38} D. Cai, X. He, X. Wu, and J. Han, “Non-negative Matrix Factorization on Manifold,” Proc. IEEE Eighth Int’l Conf. Data Mining (ICDM), pp. 63-72, 2008.
	\bibitem{b39} R. Zhi and Q. Ruan, “Discriminant Sparse Nonnegative Matrix
	Factorization,” Proc. IEEE Int’l Conf. Multimedia and Expo (ICME),
	pp. 570-573, 2009.
	\bibitem{b40} S. An, J. Yoo, and S. Choi, “Manifold-Respecting Discriminant
	Nonnegative Matrix Factorization,” Pattern Recognition Letters,
	vol. 32, no. 6, pp. 832-837, 2011.
	\bibitem{b41} N. Guan, D. Tao, Z. Luo, and B. Yuan, “Manifold Regularized
	Discriminative Non-Negative Matrix Factorization with Fast Gradient Descent,” IEEE Trans. Image Processing, vol. 20, no. 7, pp. 2030-2048, July 2011.
	\bibitem{b42} Liu, B, ``Sentiment analysis and subjectivity," Handbook of Natural Language Processing, 2, 627–666, 2010.
	\bibitem{b43} Wright, Alex. "Our sentiments, exactly." Communications of the ACM 52.4 (2009): 14-15.
	\bibitem{b44} Bollen, Johan, Huina Mao, and Xiaojun Zeng. "Twitter mood predicts the stock market." Journal of computational science 2.1 (2011): 1-8.
	\bibitem{b45} Chatterjee, Swayambhu, et al. "Classifying facts and opinions in Twitter messages: a deep learning-based approach." Journal of Business Analytics 1.1 (2018): 29-39.
	\bibitem{b46} Zhang, Yongfeng, et al. "Explicit factor models for explainable recommendation based on phrase-level sentiment analysis." Proceedings of the 37th international ACM SIGIR conference on Research \& development in information retrieval. ACM, 2014.
	\bibitem{b47} M.Conover,J.Ratkiewicz,M.Francisco,B.Goncalves,F.Menczer,and A. Flammini, “Political polarization on twitter,” in Proc. International AAAI Conference on Weblogs and Social Media, 2011.
	\bibitem{b48} Li, Stan Z., et al. "Learning spatially localized, parts-based representation." Proceedings of the 2001 IEEE Computer Society Conference on Computer Vision and Pattern Recognition. CVPR 2001. Vol. 1. IEEE, 2001.
	\bibitem{b49} Ding, Chris, Xiaofeng He, and Horst D. Simon. "On the equivalence of nonnegative matrix factorization and spectral clustering." Proceedings of the 2005 SIAM international conference on data mining. Society for Industrial and Applied Mathematics, 2005.
	\bibitem{b50} Hu, Yuheng, Fei Wang, and Subbarao Kambhampati. "Listening to the crowd: automated analysis of events via aggregated twitter sentiment." Twenty-Third International Joint Conference on Artificial Intelligence. 2013.
	\bibitem{b51} Srivatsa, Mudhakar, Sihyung Lee, and Tarek Abdelzaher. "Mining diverse opinions." MILCOM 2012-2012 IEEE Military Communications Conference. IEEE, 2012.
	\bibitem{b52} Irsoy, Ozan, and Claire Cardie. "Opinion mining with deep recurrent neural networks." Proceedings of the 2014 conference on empirical methods in natural language processing (EMNLP). 2014.
	\bibitem{b53} Liu, Pengfei, Shafiq Joty, and Helen Meng. "Fine-grained opinion mining with recurrent neural networks and word embeddings." Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing. 2015.
	\bibitem{b54} Tang, Duyu, et al. "Learning sentiment-specific word embedding for twitter sentiment classification." Proceedings of the 52nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers). 2014.
	\bibitem{b55} Weninger, Tim, Yonatan Bisk, and Jiawei Han. "Document-topic hierarchies from document graphs." Proceedings of the 21st ACM international conference on Information and knowledge management. ACM, 2012.
	\bibitem{b56} Yin, Zhijun, et al. "Latent community topic analysis: Integration of community discovery with topic modeling." ACM Transactions on Intelligent Systems and Technology (TIST) 3.4 (2012): 63.
	\bibitem{b57} Blei, David M., Andrew Y. Ng, and Michael I. Jordan. "Latent dirichlet allocation." Journal of machine Learning research 3.Jan (2003): 993-1022.
	\bibitem{b58} Cheng, Kewei, et al. "Unsupervised sentiment analysis with signed social networks." Thirty-First AAAI Conference on Artificial Intelligence. 2017.
	\bibitem{b59} Hu, Xia, et al. "Unsupervised sentiment analysis with emotional signals." Proceedings of the 22nd international conference on World Wide Web. ACM, 2013.
	\bibitem{b60} Liu, Pengfei, Shafiq Joty, and Helen Meng. "Fine-grained opinion mining with recurrent neural networks and word embeddings." Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing. 2015.
	\bibitem{b61} Yang, Bishan, and Claire Cardie. "Extracting opinion expressions with semi-markov conditional random fields." Proceedings of the 2012 Joint Conference on Empirical Methods in Natural Language Processing and Computational Natural Language Learning. Association for Computational linguistics, 2012.
	\bibitem{b62} Wang, Wenya, et al. "Coupled multi-layer attentions for co-extraction of aspect and opinion terms." Thirty-First AAAI Conference on Artificial Intelligence. 2017.
	\bibitem{b63} Fernández-Gavilanes, Milagros, et al. "Unsupervised method for sentiment analysis in online texts." Expert Systems with Applications 58 (2016): 57-75.
	\bibitem{b64} Wu, Chuhan, et al. "A hybrid unsupervised method for aspect term and opinion target extraction." Knowledge-Based Systems 148 (2018): 66-73.
	\bibitem{b65} Ibrahim, Rania, et al. "Tools and approaches for topic detection from Twitter streams: survey." Knowledge and Information Systems 54.3 (2018): 511-539.
	\bibitem{b66} Yang, Jaewon, and Jure Leskovec. "Overlapping community detection at scale: a nonnegative matrix factorization approach." Proceedings of the sixth ACM international conference on Web search and data mining. ACM, 2013.
	\bibitem{b67} Han, Jiawei, et al. "Frequent pattern mining: current status and future directions." Data mining and knowledge discovery 15.1 (2007): 55-86.
	\bibitem{b68} Friedkin, Noah E., and Eugene C. Johnsen. "Social influence and opinions." Journal of Mathematical Sociology 15.3-4 (1990): 193-206.
	
	\bibitem{t1}
	US Department of Defense, ``Joint Concept for Operating in the Information Environment (JCOIE)", July 2018.
	https://www.jcs.mil/Portals/\\36/Documents/Doctrine/concepts/joint\_concepts\_jcoie.pdf
	\bibitem{t2}
	Valeriy Gerasimov, ``Value of Science is in the Foresight'' {\em Military-Industrial Kurier\/}, Moscow, Russia, Feb 27, 2013.  (Translated from Russian by Robert Coalson:
	https://jmc.msu.edu/50th/download/21-conflict.pdf)
	
	
\end{thebibliography}
